Meanders and the Temperley-Lieb algebra

The statistics of meanders is studied in connection with the Temperley-Lieb algebra. Each (multi-component) meander corresponds to a pair of reduced elements of the algebra. The assignment of a weight $q$ per connected component of meander translates into a bilinear form on the algebra, with a Gram matrix encoding the fine structure of meander numbers. Here, we calculate the associated Gram determinant as a function of $q$, and make use of the orthogonalization process to derive alternative expressions for meander numbers as sums over correlated random walks.

==> toc.tex <==
%auto-ignore
\noindent {1.} {Introduction} \leaderfill{2} \par 
\noindent {2.} {Definitions} \leaderfill{4} \par 
\noindent \quad{2.1.} {Meanders} \leaderfill{4} \par 
\noindent \quad{2.2.} {Semi-meanders} \leaderfill{6} \par 
\noindent \quad{2.3.} {Arch configurations and (semi) meanders} \leaderfill{6} \par 
\noindent \quad{2.4.} {Walk diagrams} \leaderfill{8} \par 
\noindent \quad{2.5.} {Asymptotics} \leaderfill{10} \par 
\noindent {3.} {Temperley-Lieb algebra and meanders} \leaderfill{12} \par 
\noindent \quad{3.1.} {The Temperley-Lieb algebra and arch configurations} \leaderfill{12} \par 
\noindent \quad{3.2.} {The basis 1} \leaderfill{12} \par 
\noindent \quad{3.3.} {Scalar product and meanders} \leaderfill{14} \par 
\noindent \quad{3.4.} {Gram matrix} \leaderfill{16} \par 
\noindent {4.} {The basis 2} \leaderfill{18} \par 
\noindent \quad{4.1.} {Definition of the basis 2} \leaderfill{18} \par 
\noindent \quad{4.2.} {Properties of the basis 2} \leaderfill{20} \par 
\noindent {5.} {The meander determinant} \leaderfill{22} \par 
\noindent \quad{5.1.} {The Gram matrix for basis 2} \leaderfill{22} \par 
\noindent \quad{5.2.} {Main result} \leaderfill{22} \par 
\noindent \quad{5.3.} {The zeros of the meander determinant and their multiplicities} \leaderfill{24} \par 
\noindent \quad{5.4.} {Proof of the main result} \leaderfill{30} \par 
\noindent {6.} {Effective meander theory} \leaderfill{38} \par 
\noindent \quad{6.1.} {The matrix ${\fam \tw@ P}_n(q)^{-1}$} \leaderfill{38} \par 
\noindent \quad{6.2.} {Properties of ${\fam \tw@ P}_n(q)^{-1}$} \leaderfill{40} \par 
\noindent \quad{6.3.} {Recursion relation for the matrix ${\fam \tw@ Q}_n(q)^{-1}$} \leaderfill{42} \par 
\noindent \quad{6.4.} {The matrix ${\fam \tw@ Q}_n(q)^{-1}$} \leaderfill{46} \par 
\noindent \quad{6.5.} {The normalization matrix ${\fam \tw@ N}_n(q)$} \leaderfill{54} \par 
\noindent \quad{6.6.} {The effective theory of (semi)-meanders} \leaderfill{56} \par 
\noindent \quad{6.7.} {Connected components in meanders} \leaderfill{56} \par 
\noindent \quad{6.8.} {Asymptotics for $q \geq 2$} \leaderfill{58} \par 
\noindent \quad{6.9.} {Meander and semi-meander polynomials as SOS partition functions} \leaderfill{64} \par 
\noindent {7.} {Generalization: the semi-meander determinant} \leaderfill{68} \par 
\noindent {8.} {Conclusion} \leaderfill{74} \par 
\noindent Appendix {A.} {Proof of the formula (5.23)\ for the multiplicities of the zeros of the meander determinant} \leaderfill{74} \par 
\noindent Appendix {B.} {The Gram matrix at $q=\radical "270370 {2}$} \leaderfill{76} \par 
\noindent Appendix {C.} {Proof of the sum rule (6.41)\ } \leaderfill{78} \par 

